SPoT: Better Frozen Model Adaptation through Soft Prompt Transfer

There has been growing interest in parameter-efficient methods to apply pre-trained language models to downstream tasks. Building on the Prompt Tuning approach of Lester et al. (2021), which learns task-specific soft prompts to condition a frozen pre-trained model to perform different tasks, we propose a novel prompt-based transfer learning approach called SPoT: Soft Prompt Transfer. SPoT first learns a prompt on one or more source tasks and then uses it to initialize the prompt for a target task. We show that SPoT significantly boosts the performance of Prompt Tuning across many tasks. More remarkably, across all model sizes, SPoT matches or outperforms standard Model Tuning (which fine-tunes all model parameters) on the SuperGLUE benchmark, while using up to 27,000x fewer task-specific parameters. To understand where SPoT is most effective, we conduct a large-scale study on task transferability with 26 NLP tasks in 160 combinations, and demonstrate that many tasks can benefit each other via prompt transfer. Finally, we propose an efficient retrieval approach that interprets task prompts as task embeddings to identify similar tasks and predict the most transferable source tasks for a novel target task.

==> sections/task_transferability_OLD.tex <==
\section{Predicting task transferability}%
\label{sec:task-specific_spot}

In the previous section, we saw that \spot{} (soft prompt transfer) can significantly boost the performance of prompt tuning. However it is critical to pick the right source tasks for transfer. Through an extensive search, we found that GLUE and MNLI provide excellent source tasks for transferring to GLUE and SuperGLUE. But what about the resource-constrained scenario where a user isn't able to exhaustively search a set of source tasks? Can we \emph{predict} which tasks will best transfer onto a novel target task without testing them one by one?

To address this question, we conduct a large-scale empirical study with 26 NLP tasks (including one unsupervised task) in 160 combinations of source and target. We demonstrate that tasks can help each other via prompt transfer in various situations, and task similarity plays an important role in determining transferability. Additionally, we show that by interpreting the task prompts as task embeddings, we can construct a semantic space of tasks and formulate a more rigorous notion of task similarity. Finally, we propose a retrieval algorithm that measures task embedding similarity to choose which source tasks to use for a given novel target task (Figure~\ref{fig:approach}, right).

% Having established that prompt transfer is helpful for prompt tuning, we now turn to investigating task transferability, through the lens of task prompts. To test the transferability between different tasks, we conduct a large-scale empirical study with 26 NLP tasks (including one unsupervised task) in 160 combinations of source and target. We demonstrate that tasks can help each other via prompt transfer in various situations, and task similarity plays an important role in determining transferability. Additionally, we show that by interpreting the task prompts as task embeddings, we can construct a semantic space of tasks and formulate a more rigorous notion of task similarity. Finally, we propose a retrieval algorithm that measures task embedding similarity to choose which source tasks to use for a given novel target task (Figure~\ref{fig:approach}, right).

\subsection{Experimental setup}
\input{tbls/transfer_datasets}
We study a diverse set of 16 source datasets and 10 target datasets (see Table~\ref{tbl:transfer_datasets}).\footnote{In addition to the datasets mentioned in Section~\ref{sec:prompt_pretraining}, we also use DocNLI~\cite{WYin21}, Yelp-2~\cite{XZhang15}, CxC~\cite{ZParekh21}, DROP~\cite{DDua19}, WinoGrande~\cite{KSakaguchi20}, HellaSWAG~\cite{RZellers19}, CosmosQA~\cite{LHuang19}, RACE~\cite{GLai17}, and CR~\cite{MHu04}.}  
We consider all 160 possible source/target pairs, and perform transfer from each source task to each target task.

\subsubsection{Source and target tasks}

The source tasks comprise one unsupervised task (C4) and 15 supervised tasks covering natural language inference (NLI), paraphrasing/semantic similarity, sentiment analysis, question answering (QA), and commonsense reasoning.
All source tasks are data-rich or have been shown to yield positive transfer in prior work.
To simulate a realistic scenario, we use low-resource tasks (less than 10K training examples) as target tasks. These tasks cover the above types of tasks, and additionally include grammatical acceptability, word sense disambiguation, and coreference resolution.

\subsubsection{Training details}

To limit computational costs, we use T5 \ssc{Base} in all of our task transferability experiments.
We perform $262{,}144$ prompt tuning steps on each source task. The prompt checkpoint with the highest source task validation performance is selected to initialize prompts for different target tasks. Since the target datasets are small, we only perform 100K prompt tuning steps on each target task. We repeat each experiment three times with different random seeds. %
Other training details match those in Section~\ref{sec:training_details}.

\subsubsection{Constructing a semantic space of tasks}%
Since only prompt parameters are updated during prompt tuning on specific tasks, the learned prompts likely encode task-specific knowledge. This suggests that they could be used to reason about the nature of tasks and their relationships. To test this idea, we interpret task prompts as \textit{task embeddings} and construct a semantic space of tasks. %
More concretely, we define a task's embedding as the prompt checkpoint after training for 10K steps on that task.\footnote{Our experiments with other checkpoint alternatives yielded worse performance.} % 
Note that using early checkpoints allows for quick computation of task embeddings for novel target tasks. %
We estimate the similarity between two tasks $t^{1}, t^{2}$ by measuring the similarity between their corresponding task embeddings $\bm{e}^{1}, \bm{e}^{2}$, using the following metrics:

% While we use the best prompt checkpoints from the source tasks for transfer to the target tasks, we use earlier prompt checkpoints as our task embeddings. This enables fast computation of task embeddings for novel target tasks. %
% In our experiments, the task embedding is derived from a fixed prompt checkpoint, i.e., at 10K steps, for every task.\footnote{Our experiments with other checkpoint alternatives yielded worse performance.} %

\paragraph{\bssc{Cosine Similarity of Average Tokens}:} We compute the cosine similarity between the average pooled representations of the prompt tokens: $sim(t^1, t^2) = cos(\dfrac{1}{\bmmc{L}}\sum_{i} \bm{e}_i^{1}, \dfrac{1}{\bmmc{L}}\sum_{j} \bm{e}_j^{2})$, where $\bm{e}_i^{1}, \bm{e}_j^{2}$ denote the respective prompt tokens of $\bm{e}^{1}, \bm{e}^{2}$, and $cos$ denotes the cosine similarity.

\paragraph{\bssc{Per-token Average Cosine Similarity}:} We compute the average cosine similarity between every prompt token pair $(\bm{e}_i^{1}, \bm{e}_j^{2})$:
$sim(t^1, t^2) = \dfrac{1}{\bmmc{L}^2} \sum_{i} \sum_{j}  cos(\bm{e}_i^{1}, \bm{e}_j^{2})$.
\subsection{Predicting and exploiting transferability}
\label{sec:predict_and_exploit}
We leverage our task embeddings to predict and exploit task transferability. Specifically, we explore methods to predict the most beneficial source tasks for a given target task and then make use of their prompts to improve performance on the target task. To enlarge our set of source prompts, we use the prompts from each of three different prompt tuning runs on each source task, resulting in 48 source prompts. Given a target task $t$ with task embedding $\bm{e}^t$, we rank all the source prompts $\bm{\rho}^{s}$ in descending order by the similarity between their corresponding task embeddings $\bm{e}^{s}$ and the target embedding $\bm{e}^t$: $sim(\bm{e}^{s}, \bm{e}^{t})$. We denote the ranked list of source prompts as $\bm{\rho}^{s_r}$, where $r$ denotes the rank $(r=1,2,\ldots, 48)$. We experiment with three methods for exploiting the ranked source prompts:%

\paragraph{\bssc{Best of Top-$k$}:} We select the top-$k$ source prompts and use each of them individually to initialize the target prompt. This procedure requires prompt tuning $k$ times on the target task $t$.
The best individual result is used for evaluating the effectiveness of this method.

\paragraph{\bssc{Top-$k$ Weighted Average}:} We initialize the target prompt with a weighted average of the \mbox{top-$k$} source prompts $\sum_{r=1}^{k} \alpha_{r} \bm{\rho}^{s_r}$ so that we only perform prompt tuning on the target task $t$ once. The weights $\alpha_{r}$ are computed as $\alpha_{r} = \dfrac{sim(\bm{e}^{s_r}, \bm{e}^{t})}{\sum_{l=1}^{k} sim(\bm{e}^{s_l}, \bm{e}^{t})}
$, where $\bm{e}^{s_r}$ denotes the corresponding task embedding of $\bm{\rho}^{s_r}.
$

\paragraph{\bssc{Top-$k$ Multi-task Mixture}:} We first identify the source tasks whose prompts are in the \mbox{top-$k$} prompts and mix their datasets and the target dataset together, using the examples-proportional mixing strategy of~\citet{CRaffel20}. Then, we perform source prompt tuning on this multi-task mixture and use the final prompt checkpoint to initialize the prompt for target prompt tuning.
\subsubsection{Evaluation}
We report the average score across the target tasks achieved by using each of the methods described above. For each target task $t$, we measure the average and standard deviation of performance across the three different prompt tuning runs (which result in different task embeddings $\bm{e}^t$). For comparison, we report the absolute and relative improvements over the baseline when prompt tuning on each target task from scratch (i.e., without any prompt transfer). Additionally, we include the oracle results achieved by using a brute-force search to identify the best possible out of 48 source prompts for each target task.
\subsection{Effect of prompt-based task embeddings}
\input{figs/transfer_heatmap}
In this section, we first analyze our task transferability results. Then, we demonstrate the effectiveness of using prompt-based task embeddings for representing tasks, and for predicting and exploiting task transferability.
\paragraph{Tasks can help each other via prompt transfer in various scenarios:}  Figure~\ref{fig:transfer_heat_map} shows a heatmap of our task transferability results (see Table~\ref{transfer_results} in Appendix~\ref{appendix:transfer_results} for full results). In many cases, transferring the prompt from a source task to a target task (\textsc{source~$\rightarrow$~target}) can provide significant gain on the target task. The transfer MNLI~$\rightarrow$~CB yields the largest relative error reduction of 58.9\% (from an average score of 92.7 to 97.0), followed by MNLI~$\rightarrow$~COPA (29.1\%) and ReCoRD~$\rightarrow$~WSC (20.0\%). Using the best source prompt (out of 48) for each target task dramatically improves the average score across 10 target tasks from 74.7 to 80.7. Overall, our results show effective transfer from large source tasks that involve high-level reasoning about semantic relationships among sentences (e.g., MNLI), or when the source and target tasks are similar (e.g., CxC~$\rightarrow$~STS-B). Interestingly, positive transfer can occur in cases where the tasks are relatively dissimilar (e.g., ReCoRD~$\rightarrow$~WSC, SQuAD~$\rightarrow$~MRPC, CxC~$\rightarrow$~WiC).\footnote{Table~\ref{effective_transfers} in Appendix~\ref{appendix:transfer_results} contains more cases.} %
\input{figs/fig4}
\input{figs/fig6}
\paragraph{Task embeddings capture task relationships:}
Figure~\ref{fig:task_clustermap} shows a hierarchically-clustered heatmap of cosine similarities between the task embeddings of the 26 NLP tasks we study using the \ssc{Cosine Similarity of Average Tokens} metric.\footnote{To obtain the highest resolution of similarity between two tasks, we use the average of cosine similarities between their task embeddings obtained with all the three different prompt tuning runs (9 combinations).} 
We observe that our learned task embeddings capture many intuitive task relationships. Specifically, similar tasks are grouped together into clusters, including question answering (SQuAD, ReCoRD, and DROP; MultiRC and BoolQ), sentiment analysis (Yelp-2, SST-2, and CR), NLI (MNLI and CB; DocNLI and RTE), semantic similarity (STS-B and CxC), paraphrasing (MRPC and QQP), and commonsense reasoning (WinoGrande, HellaSWAG, and CosmosQA). We note that QNLI, which is an NLI task built from the SQuAD dataset, is not closely linked to SQuAD; this suggests that our task embeddings are more sensitive to the type of task than domain similarity. %
Interestingly, they also capture the unintuitive case of ReCoRD's high transferability to WSC\@. Additionally, task embeddings that are derived from different prompts of the same task have high similarity scores (see Appendix~\ref{appendix:task_embedding_similarity}).
\paragraph{Correlation between task embedding similarity and task transferability:} Figure~\ref{fig:similarity_vs_transferability} shows how the relative error reduction on a target task changes as a function of the similarity between the source and target task embeddings. Overall, we find that there is a significantly positive correlation between task embedding similarity and task transferability on four (out of 10) target tasks we study, including STS-B ($p < 0.001$), CB ($p < 0.001$, not shown) %
, WSC ($p < 0.01$), and RTE ($p < 0.05$), while it is less significant on the other tasks.
\paragraph{Task embeddings can be used to predict and exploit task transferability:} We compare the results of different methods for identifying which source prompts could be beneficial for a given target task in Table~\ref{tbl:predict_transferability}.
We find that using the \ssc{Per-token Average Cosine Similarity} metric yields better results than using the \ssc{Cosine Similarity of Average Tokens} metric for small values of $k$ ($\leq 9$). Our results also suggest that \ssc{Best of Top-$k$} provides an effective means of predicting and exploiting task transferability. Simply choosing the source prompt whose associated task embedding has the highest similarity to the target embedding using the \ssc{Per-token Average Cosine Similarity} metric improves over the baseline by a large margin (from an average score of 74.7 to 76.7, a 12.1\% average relative error reduction).
Trying all the top-3 (out of 48) source prompts for each target task yields an average score of 77.5.
With larger values of $k$, we can retain most of the benefits of oracle selection of source prompts %
(80\% of the gain in terms of average score with $k=9$ and 90\% with $k=15$), while still eliminating over 2/3 of the candidate source prompts. Although this approach requires prompt tuning on the target task $k$ times, the cost of prompt tuning is relatively inexpensive, compared to model tuning. \ssc{Top-$k$ Weighted Average} has similar average performance to \ssc{Best of Top-$k$} with $k=1$, but achieves lower variance. Thus, this may be an appealing alternative to \ssc{Best of Top-$k$} in scenarios where multiple tuning runs on the target task are prohibited. Finally, \ssc{Top-$k$ Multi-task Mixture} also provides a means of obtaining strong performance with an average score of 77.8, even outperforming \ssc{Best of Top-$k$} with $k \leq 3$.
\input{tbls/predicting_transferability}




